$\ell^2$ Betti numbers and coherence of random groups

We study $\ell^2$ Betti numbers, coherence, and virtual fibring of random groups in the few-relator model. In particular, random groups with negative Euler characteristic are coherent, have $\ell^2$ homology concentrated in dimension 1, and embed in a virtually free-by-cyclic group with high probability. Similar results are shown with positive probability in the zero Euler characteristic case.

==> Figure_SmallCancellation.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.9,>=latex,decoration={
    markings,
    mark=at position 0.6 with {\arrow{>}}}]
% Axis at left hand side
\begin{scope}[gray!90]
\begin{scope}[shift={(-7.5,0)}]
\draw[->] (0,-3.5)--(0,1) ;
\end{scope}
\draw[dotted] (-6.3,0)--(4,0); 
\draw[dotted] (-4.5,-2)--(4,-2); 
\draw[dotted] (-4.5,-3)--(4,-3); 
\end{scope}
\begin{scope}[gray!120]
\draw (-7.5,1) node[above]{$\phi,\psi$};
\draw (-6.85,0) node[]{$\phi_{\rm min}$};
\draw (-6,-2) node[]{$\phi_{\rm min}-\frac{N(N-1)}{2}$};
\draw (-6,-3) node[]{$\phi_{\rm min}-\frac{N(N+1)}{2}$};
\end{scope}
%Initial arrows
\draw[postaction={decorate}] (-4,1.5) -- (0,0) node[midway,above]{$\ttx_n$};
\draw[postaction={decorate}] (0,0) -- (4,1) node[midway,above]{$\ttx_i$};


%Parts of w_n
\begin{scope}[red]

\draw[postaction={decorate}] (-2.5, -2) -- (-1.5,-2) node[midway, below]{$\tty_1^{n-m+1}$} ;
\draw[postaction={decorate}] (-1.5,-2) .. controls (-1.3,-0.8) and (-0.3,-0.1).. (0,0);
\draw[postaction={decorate}] (-4,0) .. controls (-3.7,-0.1) and (-2.7,-0.8) .. (-2.5,-2);
\draw[postaction={decorate}] (-4,1.5) -- (-4,0) node[midway, left]{$\ttz^{-\phi(\ttx_n)}$};
%\draw[dashed, postaction={decorate}] (-3.9, 1.3) ..controls (-3.9,0.8) and (-3.9,0.4)..(-3.7,0.2)-- (-3.3,-0.2)..controls (-3.1,-0.3) and (-2.5, -1.5)..(-2,-1.5)..controls (-1.5,-1.5) and (-1.6,-1.2).. (-1.4,-1).. controls (-1.3,-0.8) and (-0.8,0)..(-0.3,0);
\draw (-2,-1.2) node[above]{$w_n$};
\draw[dashed, postaction={decorate}] (-2.5,-0.9) arc (-170:0:0.5);
\end{scope}
%Parts of w_i

\begin{scope}[red]

\draw[postaction={decorate}] (1.5, -3) -- (2.5,-3) node[midway, below]{$\tty_i$} ;
\draw[postaction={decorate}] (0,0) .. controls (0.3,-0.1) and (1.3,-0.8) .. (1.5,-3);
\draw[postaction={decorate}] (2.5,-3) .. controls (2.7,-0.8) and (3.7,-0.1) .. (4,0);
\draw[postaction={decorate}] (4,0) -- (4,1) node[midway, right]{$\ttz^{-\phi(\ttx_i)}$};
%\draw[dashed, postaction={decorate}] (-3.9, 1.3) ..controls (-3.9,0.8) and (-3.9,0.4)..(-3.7,0.2)-- (-3.3,-0.2)..controls (-3.1,-0.3) and (-2.5, -1.5)..(-2,-1.5)..controls (-1.5,-1.5) and (-1.6,-1.2).. (-1.4,-1).. controls (-1.3,-0.8) and (-0.8,0)..(-0.3,0);
\draw (2,-1.7) node[above]{$w_i$};
\draw[dashed, postaction={decorate}] (1.5,-1.4) arc (-170:0:0.5);
\end{scope}
\end{tikzpicture}
\caption{A schematic showing the replacement of $\ttx_i$ with $w_i$ at the minimum point of a relator $r_i$. The `parabolic' segments represent those parts of the words $w_i$ and $w_n$ not otherwise labelled. The vertical scale shows the variation of $\phi$ and $\psi$ over the words. The horizontal scale has no precise meaning.}
\label{fig_SmallCancellation}
\end{figure}
